The Road Not Taken: Re-thinking the Feasibility of Voice Calling Over Tor

Anonymous VoIP calls over the Internet holds great significance for privacy-conscious users, whistle-blowers and political activists alike. Prior research deems popular anonymization systems like Tor unsuitable for providing requisite performance guarantees that real-time applications like VoIP need. Their claims are backed by studies that may no longer be valid due to constant advancements in Tor. Moreover, we believe that these studies lacked the requisite diversity and comprehensiveness. Thus, conclusions from these studies led them to propose novel and tailored solutions. However, no such system is available for immediate use. Additionally, operating such new systems would incur significant costs for recruiting users and volunteered relays, to provide the necessary anonymity guarantees. It thus becomes imperative that the exact performance of VoIP over Tor be quantified and analyzed so that the potential performance bottlenecks can be amended. We thus conducted an extensive empirical study across various in-lab and real-world scenarios to shed light on VoIP performance over Tor. In over 0.5 million measurements spanning 12 months, across seven countries and covering about 6650 Tor relays, we observed that Tor supports good voice quality (Perceptual Evaluation of Speech Quality (PESQ) >3 and oneway delay <400ms) in more than 85% of cases. Further analysis indicates that in general for most Tor relays, the contentions due to cross-traffic were low enough to support VoIP calls, that are anyways transmitted at low rates (<120 Kbps). Our findings are supported by concordant measurements using iperf that show more than the adequate available bandwidth for most cases. Data published by the Tor Metrics also corroborates the same. Hence, unlike prior efforts, our research reveals that Tor is suitable for supporting anonymous VoIP calls.

==> abstract.tex <==
\section{Abstract}
Anonymous VoIP calls over the Internet remains a pipe dream for privacy conscious users, whistle-blowers and political activists alike. 
The scant prior research deems popular anonymization systems like Tor unsuitable for providing requisite performance guarantees
that real-time applications like VoIP need. Their claims are backed
by results based on studies that lacked diversity or involved pessimistic experimental setups. 
Biased by such conclusions, some of them proposed novel and tailored solutions.
Interestingly no such system currently exists.
Moreover, for such system to operate it would incur significant costs for recruiting users
and volunteered relays, so as to provide the necessary anonymity guarantees.
 
It thus becomes imperative that the exact performance of VoIP over Tor be quantified and analyzed, so that
the (potential) performance bottlenecks can be amended. Sadly, the prior efforts ignored quantifying
the impact of interplay of the network performance attributes
(\emph{e.g.} RTT, bandwidth \emph{etc.}) on the perceived call quality.
We thus conducted an extensive empirical study across various in-lab and real world scenarios to shed light on VoIP performance over Tor. In over 0.5 million measurements spanning 18 months, across 7 countries and covering about 6650 Tor relays, we observed that \textit{Tor supports good voice quality (PESQ \textgreater 3 and one-way delay \textless $400ms$) in more than 85\% of
cases}. Further analysis indicate that in general for most Tor relays, the contentions due to cross-traffic were
low enough to support VoIP calls, that are anyways transmitted at low rates (\textless 120Kbps).
Our findings are supported by concordant measurements using \texttt{iperf} that show more than
adequate available bandwidth for most cases. This is backed by data published by Tor Metrics.
Hence, contrary to all prior efforts, our results show that Tor is suitable for making anonymous VoIP calls

==> analysis_old.tex <==
\section{Insights from Measurements}
\label{analysis}
In this section we present explanation of the aforementioned results, along with other interesting insights we observed from our results.


\subsection{Correlation with bandwidth}
\textcolor{blue}{SC: Need to rethink the subsection heading}
Computing PESQ involves comparison of the
original audio clip, as played out by the caller, and
the audio recorded at the callee. 
Decrease in bandwidth, normally increases
chances of packet drops and delays. 
On the other hand, increase in bandwidth,
reduces such chances. Thus, 
such drop and delays may predictably
vary PESQ, which relies on error
free reception of voice packets
at the callee.


On an average we observed a high PESQ and acceptable OWD
where the available bandwidth of a Tor
circuit was high.
For \emph{e.g.} in about 90\% across all
our experiments, we observed over 1 Mbps
available bandwidth. In 94\% of these high bandwidth cases PESQ was
greater than 3, with the mean being $\approx$ 3.9.
The corresponding average OWD was about XXXXms.




%we observed 
%PESQ of 3.9 for circuits whose whose average
%bandwidth was \textgreater 1 Mbps, with about 94\% of these recording PESQ \textgreater 3.
%Here the OWD was about XXXX..

Conversely, we observed low PESQ and/or unacceptably high
OWD in case the available bandwidth was low. 
For \emph{e.g.} in about 3\% of all
the cases we observed less than 500 Kbps
bandwidth. About 25\% of these cases recorded
PESQ \textless 3, with the mean being 3.45. More importantly the average
OWD shout up to 461ms (15\% higher than
acceptable limit).



%when available
%bandwidth was \textless 500 Kbps, the average PESQ was 3.45,
%with about 25\% having PESQ \textless 3. More importantly
%the average OWD shot up to 461ms, \emph{i.e.} about 15\% higher
%than the acceptable limit.

\textcolor{blue}{SC: Probably a paragraph/noindent separation}

Good call quality in an overwhelming majority of the
cases can be attributed to the fact that popular codecs, designed for VoIP~\cite{}, encode
voice mostly at relatively low (constant) bit rates (\textless 200 Kbps).
The delays and losses in voice traffic, as recorded by the callee,
is reasonably low for majority of the Tor circuits, due to the adequate bandwidth.




%In our experiments, we observed \textgreater 1Mbps available bandwidth for about 90\% of our Tor circuits, 
%while only around 3\% observed bandwidth \textless 500Kbps. 
%The remaining were between 500Kbps and 1Mbps.
%Such high bandwidths, result in relatively l

%are sufficient
%to transport encoded voice with adequate call quality.
Moreover, such high available bandwidths corroborate
with observations reported by the Tor Metrics (TM) project~\cite{tormetrics}.
TM reports an average available bandwidth of $\approx1.6$Mbps
while downloading a 1MiB file.


\textcolor{blue}{You may need a subsubsection heading}
However, contrary to our expectation, in about X\% cases we observed
poor call quality even with available high bandwidth. For \emph{e.g.},
in these cases we observed an average PESQ of 2.4 when then bandwidth was \textgreater 3.
%Upon investigation we observed
%an interesting phenomenon related to PESQ. 


To identify the root cause of such observations we tried
to re-create such scenarios, \emph{i.e.} high available
bandwidth and low call quality, through a V-Tor in-lab setup: 
\begin{enumerate}
    \item We setup a bottleneck link of 10Mbps between the caller and a callee, and the callee also ran a webserver.
    
    \item The caller instantiated a single call and captured the traffic using \texttt{pcap}.
    
    \item After about 10s, the caller also started 10 parallel TCP wgets downloading a large file from the webserver (hosted on the callee machine). In steady state each of these flows received $\approx$ 1Mbps. Here we observed an interesting phenomenon. 
    The call traffic suffered significant losses, coincident with the arrival of the
    several parallel \texttt{wgets}s (as observed from the \texttt{pcap}).
    Eventually the \texttt{wget}s were terminated once the call ended.
    
    \item For this test, we observed a PESQ \textless 3 in around x\% of the cases.
    
    \item Quantum increases in the number of parallel wgets (from 10 to 50, adding 10
    connections each time), led to progressive degradation of PESQ at each step.
    In the worst case, the PESQ was never over 3. However, here each of the 
    \texttt{wget} flows received $\approx$ 200 Kbps, indicative of requisite bandwidth. 
 
    \item We observed a similar trend even when the bottleneck bandwidth was 100 Mbps.     
\end{enumerate}

This shows that, an increase in contentious cross-traffic, despite sufficient available bandwidth for a call (\textgreater 100Kbps), degrades PESQ progressively, particularly
in the presence of high traffic contention. 

Upon further inspection of the \texttt{pcap} traffic captures, corresponding to these calls, we observed 
that even minor loss or delay of packets carrying voice traffic, at the receiver, led to significant reduction of measured PESQ. 

More specifically, in the majority cases
($\approx$ 94\%) measured bandwidth (using
iperf) and PESQ varied monotonically.

More specifically, in majority of the cases with
high available bandwidth (\textgreater 1Mbp), 
we observed PESQ of 3.9.


For \emph{e.g.} drop in available
bandwidth from over 1Mbps to less than 500 Kbps dropped PESQ from 3.9 
to about 3.45. In about 6\% of these cases, while observed the opposite.
For \emph{e.g.} when available bandwidth was about 1 Mbps, PESQ was 2.4.
PESQ is sensitive to losses and delays. Minor variations in these
parameters is easily captured by PESQ. Thus in these divergent cases
clearly the losses and delays was higher, even with high measured bandwidth.

There are possible multiple explanations of this phenomenon, some of which
are more likely than others:
\begin{enumerate}
    \item \texttt{Iperf} measures available bandwidth in terms
    of bytes/bits transferred over the course of the test, but fails
    to capture other events like losses and delays, which actually 
    have a sharp impact on PESQ.
    
    
    \item High available bandwidth, but less space available in the path bottleneck queue to
    buffer the voice packets.
    
    
    
    \item High congestion due to cross-traffic, highly coincident only with our voice calls (but not at other times). 
    
     
\end{enumerate}
    





Increasing losses progressively degrade PESQ (as shown in Fig.~\ref{}). 
We observed a similar behavior even upon analysing the \texttt{pcap} for
experiments for public Tor network.

%Infact, such losses corroborated with coincident audible glitches.

Hence, it appears, that poor performance despite adequate
bandwidth, can be only attributed to contention
either due to high cross-traffic volume or 
low available buffer capacity of the bottleneck
link, or both. This may cause packet drops or delays.
While such drops or delays may not have much impact
on the users' web browsing experiences, it may signifiantly impact
the perceived quality (PESQ score) of real-time voice. 


% Augmenting the above findings, we observed that the fraction of calls getting an average bandwidth of $>1$Mbps was around 90\% and only 3\% calls observed average bandwidth $<500Kbps$, explaining the reason for the overall good performance of VoIP calls, given the correlation of call quality with bandwidth. A point to note is that, this available bandwidth we get for calls is in accordance with the data provided by the Tor metrics (TM) project~\cite{tormetrics}. The TM reports that for downloading a 1MiB file, they obtained $\approx1.6$Mbps bandwidth.

% It is important to highlight the fact that none of the existing literature (which evaluated voice quality over Tor or which build new architectures and systems) has reported such a finding.

\begin{figure}[h]
\centering
%\vspace{0.25cm}
\includegraphics[scale=0.32]{fig/PESQ_BW_bar.pdf}
\caption{\normalsize{PESQ vs Bandwidth}}
\label{PESQ_BW}
\end{figure}

\begin{figure}[h]
\centering
%\vspace{0.25cm}
\includegraphics[scale=0.32]{fig/OWD_BW_bar.pdf}
\caption{\normalsize{OWD vs Bandwidth}}
\label{OWD_BW}
\end{figure}





\subsection{Coverage Over Tor}
%This section deals with all the analysis related to the Tor circuits we created, the number of unique relays we got, the overall Tor nodes coverage in our experiments etc. As previously explained in Sec. xx, we recorded the Tor circuit of all the calls performed over Tor.  We aggregated that data and analysed these circuits to reveal out interesting facts about our study.

We recorded and analysed Tor circuit information for all our experiments.
We now present some interesting insights we observed from this analysis.

A total of 400,000 Tor circuits were created during our study.
%spread aross $7$ countrie.
These circuit involved a total of 6650 unique Tor relays.
Prior research (Rizal \emph{et al.}~\cite{rizal2014study}) reportedly used
only 250 relays, that too restricted to Europe.

%Note that none of the previous literature was able to provide a comprehensive coverage of Tor nodes (max 250 by Rizal et al.). 
%In our study we covered almost 6650 relays and hence this study can be considered representative of the overall quality one might expect when initiating voice calls over Tor.

%The reason for such coverage can be attributed to the Tor circuit selection algorithm which does not depend on geography, rather on bandwidth weights. Further, the relay selection algorithm makes sure than no few nodes are provided all the Tor traffic, while rest are starving for new connections.

Moreover, we also observed that the top-10 relays, sorted by measured bandwidth, appeared most often in the circuits. For \emph{e.g.}, IPreadtor~\cite{}, the relay with highest bandwidth across all the relays was selected most often, \textit{i.e.} 2464 times.


%did a frequency analysis of these relays and found out that the top 10 relays with the maximum bandwidth were roughly selected the maximum number of times. For example IPreadtor~\cite{}, the relay with highest bandwidth across all the Tor relays was selected the most number of times \textit{i.e.} 2464.

%None of the previous literature was able to provide a comprehensive coverage of Tor nodes (max 250 by Rizal et al.). In our study we covered almost 6650 relays and hence this study can be considered representative of the overall quality one might expect when initiating voice calls over Tor.


==> intro-backup.tex <==
\section{Introduction}
%Users have been concerned about communication privacy from a long time~\cite{} leading to the development of a lot of secure (end to end encrypted) and private communication applications such as Signal~\cite{}, Telegram~\cite{} etc. The need for communication privacy has been extended to VoIP leading to the development of secure VoIP calling apps. However, there are a lot of instances involving the nation state and organizations like FBI
With the advent of Voice-over-IP (VoIP) applications and their support for encrypted traffic, VoIP apps have gained popularity among regular users as well as those who are concerned about their communication privacy. However, for Internet clients residing in dictatorial regimes, which conduct mass surveillance, existing VoIP systems fail to ensure anonymity of the users (for example, the ability of NSA to intercept Skype conversations is widely known~\cite{verizon,nsaprismskype}). Moreover, there does not exist any ubiqitous system that guarantees confidentiality and anonymity required for regular Internet users, whilstleblowers
and political activists alike.

%Rather, there does not exist a single solution which guarantees both confidentiality and anonymity to the VoIP users --- regular Internet clients, whistleblowers and political activists (for example, the ability of NSA to intercept Skype conversations is already known). }
%Moreover, there does not exist any ubiqitous system that
% provides the real time communication anonymity and privacy required for regular Internet users, whilstleblowers
% and political activists alike.

% Anonymous censorship resistant communication systems are primarily designed
% keeping in mind semi real-time applications like web browsing. Such 
% systems mostly involve rerouting (potentially
% monitoried or filtered) network traffic via proxies (either individual or cascade).
% One such system, Tor~\cite{syverson2004tor}, has gained prominence as the \emph{de-facto}
% anonymity preserving censorship resistant system and often used by
% journalists and whilstle-blowers globally \textcolor{red}{cite}. Mobile application
% revolution has augmented the whistle-blowers' arsenal
% with real time communication apps (\emph{e.g.} those supporting
% real-time audio and videoconferencing). 
% \textcolor{red}{We require motivation for anonymous call..}
% \textcolor{blue}{SC: Piyush please add as per our discussion...}
On the other hand, for existing anonymity based systems
like Tor, it is believed that, rerouting traffic via circuitous paths,
potentially incur unwanted latency for real-time applications like
VoIP. Further, while traditionally VoIP
relies on UDP traffic to ensure real-time guarantees,
most such proxying systems are designed to transport
TCP. 
Moreover, complex cryptographic handshakes
and signatures, essential to the anonymity guarantees provided by such systems, 
may exacerbate the already pathological situations.
\textcolor{blue}{MM: This line is not clear, what do you mean by pathological situation?}


%,ccs10-scheduling} 
%and are thus an additional
%source of unacceptable delays  \textcolor{red}{This is fixed by KIST, We can even highlight that solutions like KIST are supposed to improve the overall performance of Tor} . Finally, complex cryptographic handshakes
%and signatures, essential to the censorship resistance
%and anonymity guarantees provided by such systems, 
%\textcolor{red}{may} exacerbate the already pathological situations \textcolor{red}{There is not much evidence for this}. 

Almost all past efforts~\cite{danezis2010drac,le2015herd,heuser2017phonion,schatz2017reducing} unequivocally agree upon 
such narratives , with a few providing 
negligible empirical evidences or explanations
supporting such claims~\cite{rizal2014study,heuser2017phonion}.
Hence, the current literature propose building new architectures and systems~\cite{le2015herd,heuser2017phonion,danezis2010drac}. But none of the proposed solutions are functional and available for use at present.
%\textcolor{red}{and propose building new architectures and systems}

%\textcolor{red}{Moreover, none of the proposed solutions are functional and available for use at present.}

 %ITU guidelines dictate various network parameters (\emph{e.g.} PESQ, One-way delay \emph{etc.}) for acceptable VoIP quality. 
%  Most existing efforts \textbf{Cite DRAC, Torphone, Rizal, Herd and Phonion} seem to either rely
%  on the premise that Tor circuits incur unacceptable overheads on such parameters and 
%  propose building novel architectures that provide the requisite
%  performance guarantees. 
% However there are some fundamental problems with all such proposals.  
 

%Some~\cite{rizal2014study,heuser2017phonion} merely report 
%\textcolor{red}{through a few hundred voice calls}
%that the traffic over Tor does not meet such criteria. 
%\textcolor{red}{but these studies are limited due to either very less Tor coverage (250 by Rizal and 300 max by Phonion) or by}.
%They even propose building novel architectures that
%provide the necessary performance guarantees. 

Additionally, recently proposed systems like Phonion and Herd requires a new volunteer run network 
along with millions of active users
(like Tor) for their functioning. This requirement can be a major stumbling block for these systems to scale. 
Moreover, in the absence of active users and insignificant
cross-traffic, comparable to that of Tor (that supports over
2 million users and transports over 150Gbit/s traffic per day~\cite{tor-metrics})
, one cannot adjudge future real-world anonymity and performance
assurances of these proposed systems. 

Also, there seem to be conflicting evidences
in the existing literature, \emph{w.r.t} empirically
measured parameters like RTT with Herd reporting an RTT of 2-4s whereas Ting~\cite{cangialosi2015ting} in the same year claimed that in thousands of circuits, they did not observe an RTT $>1s$ for 3-hop circuits. Further,
prior research efforts neither quantify the exact interplay of the various network
parameters involved,
nor explain how that results in poor voice call quality.\textcolor{blue}{MM: place this para before the previous one}

Hence, in the absence of (1) comprehensive performance analysis of VoIP calls over Tor; and (2) available
anonymous VoIP communication systems, we chose to
determine as to why VoIP performs poorly over Tor, such that it could be improved accordingly, resulting in an immediately usable system.
We thus began by initiating VoIP calls through Tor
and contrary to previous studies we found that 
%in an initial attempt 
out of 1000 calls, 80\% calls were of acceptable call quality.

% in various in-lab and real-world
% setups, involving diverse Tor relays, network media, VoIP application and 
% peers dispersed across $7$ countries..
% Our objective was to observe the interplay between
% network parameters that resulted in poor call quality.
% Even after XXX calls, transported via random Tor
% circuits (created via the Tor client program), we
% failed to find enough instances (less than XXX) where the performance
% was poor (PESQ < XXX). 


Thereafter we conducted a large scale and extensive longitudinal study involving 0.5 million voice calls over the Tor network, spanning
over 1.5 years. 



These tests involved varied in-lab and real world scenarios with diverse Tor relays, network media, VoIP applications with caller and callee dispersed across 7 countries and 3 continents. 
To our
surprise, even with such diverse measurements, more than 90\% of voice calls performed considerably well, 
with PESQ $>3$ and OWD $<400ms$ (considered acceptable as per ITU guidelines~\cite{itu2003recommendation,itu2000g}). 

We then investigated the reason for such an overwhelmingly large set of good quality calls. We observed that the tested VoIP applications 
%(pjsip~\cite{} and Mumble~\cite{})
transmit voice at a constant and low bitrate generally $<120Kbps$ 
%(including the overhead of sending it over Tor)
\footnote{This holds true for standard SIP based apps and non-SIP based apps such as Telegram and Skype.}. In 90\% of the cases we recorded the available bandwidth in the call circuits to be $>1Mbps$ which show a high correlation to the observed performance. This observation of majority circuits getting adequate bandwidth is in accordance with the data provided by the Tor metrics project. 
%However, the impact of this data, was not studied in context of VoIP calls.  
%In Sec.~\ref{} we explain this phenomenon in much more detail.

%as the bandwidth requirements for VoIP
%applications is low, and 
%contentions with cross traffic not significant.

%Upon further investigation, we discovered that
%VoIP calls, which by and large require no more
%than 100 Kbps of available bandwidth, were successfully transported via Tor circuits without much distortions. We attribute this
%to the available bandwidth in Tor relays.

Our research is the first study that involves extensive empirical
evaluation of the performance of VoIP over Tor. We summarize the contributions as follows :
\textcolor{blue}{MM: can we share the insights here?}
%We summarize findings of our longitudinal comprehensive evaluation through the following important findings:
\begin{enumerate}
    \item In vast majority of our experiments, we observed good call quality with PESQ over 3 and OWD under 400ms. This holds true for diverse set of experiments involving :
    \begin{enumerate}
        \item Caller and Callee spread across 7 countries.
        \item Coverage of 6650 Tor relays.
        \item Wired, WiFi and 4G environment.
        \item Popular apps such as Telegram and Skype.
        \item One way and Two way anonymity.
        \item Various codecs and call duration.
    \end{enumerate}
    \item Such acceptable performance is primarily due to
    the available bandwidth across vast majority (\textgreater $99\%$) of 
    public Tor relays, and low cross-traffic contentions with VoIP flows.
    Popular VoIP applications transmit traffic at low constant bit rates
    and available bandwidth in relays is adequate to support such flows. 
\end{enumerate}

Overall, we observed that in vast majority of Tor circuits
\emph{one can expect reasonable call quality as packet drops, due
to contentions with cross traffic is not significant; the VoIP call
codecs do not require much bandwidth anyways}.
Hence, contrary to all previous research conclusions, we believe
that Tor seems to be a suitable infrastructure
that could be used for transporting VoIP traffic.

%These tests were varied over space and time spanning across $7$ countries over a duration of $1.5$ years

%. Such
%systems, unlike Tor, cannot provide adequate
%anonymity guarantees due to the lack of users
%that existing deployed systems like Tor have. 
%Moreover, there are no current functional implementations Herd. 

%In the absence of available systems, we chose
%to investigate exactly \emph{why Tor provides inadequate guarantees for VoIP.}, so as to
%determine how to improve the performance guarantees
%for VoIP. 



%\textcolor{red}{
%However to our surprise, even after we conducted comprehensive

%tests --- over 500,000 voice calls
%consisting of various .}

%in less than \textbf{XXX}$\%$ of these tests
%VoIP performed poorly (PESQ $<XXX$).

% Overall, in vast majority of our experiments across all scenarios
% we observed reasonable performance of VoIP
% calls with PESQ $>3$ and One Way Delay (OWD) $<400ms$ over Tor. 








%ITU guidelines dictate
%that the following performance requirements for
%transporting VoIP traffic without significant degradation
%in perceived quality.

%\begin{enumerate}
%    \item Acceptable on-way delay: XXXms.
%    \item Jitter:....
%    \item Packet losses:....
%\end{enumerate}
    
    
    









%The reader might 





%In our research we consider two different kinds of
%adversaries --- A censorious nation-state level adversary
%which may observe, record and filter VoIP traffic by
%influencing the ISPs within its jurisdiction. The
%other, adversary is a more powerful nation-state adversary 
%that apart from merely observing and filtering VoIP
%traffic may coerce VoIP service providers to reveal
%the user identities, their login times and call duration
%and may use such information to augment their censorship
%activities. 

%Our research involved studying the two types

% \textbf{***************************************}
% --The big question: Can we achieve anonymous VoIP calling?

% --Existing literature talks about a lot of solutions, but those are all prototypes and there is no deployable or readily available solution yet for doing anonymous call

% --Obvious selection is Tor (as it is maintained actively) , but is believed not to be suitable because of its performance bottlenecks and the delay it incurs [citations].

% --Hence, in order to make anonymous calling deployable we started with trying to find out performance bottlenecks in Tor with respect to voice calls, so that they might be patched.

% --We did an initial performance analysis and got decent results which were surprising as the existing literature believed Tor to not be suitable for the same.

% --Here we felt a gap, as there was no measurement study which did a large scale empirical analysis of voice calls over Tor. All we had was a few 100 calls by two of the authors, which were not sufficient to tell the complete picture.

% --Therefore, we launched a large comprehensive measurement campaign and found out that anonymous calling is indeed possible over Tor with some interesting findings.

% Challenge: efficiently sending UDP packets inside TCP packets; understandable by Tor;

% Two different setups were used M-Tor/V-Tor;

%     Imp. findings.....




==> limitations.tex <==
\section{Future Work}
\label{future}
We list the possible future work :

\begin{itemize}
    \item We are currently working on building a measurement platform which will consistently keep initiating voice calls over Tor and report the corresponding results over time. We plan to store this data so that it can be analysed and used for future research purposes.
    \item Although M-Tor is easy to setup as it is a GUI based system, V-Tor involves quite a lot of steps as it requires to configure SIP server and a VPN server. Also, currently there does not exist a portable solution of our M-tor setup for performing anonymous calls across every platform. Hence, in future we plan to create standalone software bundles for client as well as servers. 
    \item We plan to explore the possibility of performing conference calls and analyse their call quality. Further, given that Tor provides $>1Mbps$ bandwidth in a majority of its circuits we plan to empirically study the performance of video streaming over Tor.
    \item Lastly, we evaluated the performance of a few popular apps such as Telegram and Skype. In future we plan to investigate in detail the performance of other popular applications such as Whatsapp, Google Hangouts etc.
\end{itemize}


% 1. Prototype for easy setup
% 2. evaluating other 3rd party apps
% 3. Conference calls,video calls
% 4. Measurement platform for consistently measuring quality of 5. VoIP calls over Tor, something like tor metrics.




==> threatmodel.tex <==
\section{Threat Model}
\textcolor{blue}{Put this under Types of Anonymous calling, or in measurement approach section?}

We consider two types of adversaries for our system. Our first adversary is a  nation-state, that analyze network flows of its countries. The adversary can monitor Internet traffic using any known technique (DNS injection, IP address/URL filtering, DPI, \emph{etc.}), and may also monitor and manipulate network packets that cross its boundaries --- \emph{e.g.} dropping or delaying some packets in an attempt to detect/disrupt anonymous communication systems --- but we assume it is \emph{not} willing to completely block all Internet traffic.

Additionally, we also consider a second adversary which is a \textit{powerful} nation state, that in addition to the capabilities of first adversary, might also coerce third-party organizations (within/outside its jurisdiction) to reveal information of suspected clients. For example, a censorious government might pressurize organizations like Skype, WhatsApp, Telegram \emph{etc.,} to reveal information about suspected VoIP clients.


